Multimodal Speech Recognition for Language-Guided Embodied Agents

Benchmarks for language-guided embodied agents typically assume text-based instructions, but deployed agents will encounter spoken instructions. While Automatic Speech Recognition (ASR) models can bridge the input gap, erroneous ASR transcripts can hurt the agents' ability to complete tasks. In this work, we propose training a multimodal ASR model to reduce errors in transcribing spoken instructions by considering the accompanying visual context. We train our model on a dataset of spoken instructions, synthesized from the ALFRED task completion dataset, where we simulate acoustic noise by systematically masking spoken words. We find that utilizing visual observations facilitates masked word recovery, with multimodal ASR models recovering up to 30% more masked words than unimodal baselines. We also find that a text-trained embodied agent successfully completes tasks more often by following transcribed instructions from multimodal ASR models. github.com/Cylumn/embodied-multimodal-asr

==> Objects/tab_dataset_counts.tex <==
\begin{table}[th]
  \centering
  \setlength{\tabcolsep}{5pt}
  \caption{Spoken instruction and household scene counts in our benchmark derived from the ALFRED text instructions.}
  \begin{tabular}{ lrrrr }
    &{\textbf{Train}} & {\textbf{Validation}} & \multicolumn{2}{c}{\textbf{Test}}\\
    &                 &                  & {\textit{Seen}} & {\textit{Unseen}} \\
    \toprule
    \# Instructions & 41,474 & 5,222 & 5,570 & 5,140 \\
    \# Scenes & 108 & 87 & 88 & 4 \\
    \bottomrule
  \end{tabular}
  \label{tab:dataset_counts}
  
\end{table}

==> Objects/tab_mask_counts.tex <==
\begin{table}[t]
  \setlength{\tabcolsep}{3.5pt}
  \caption{Percentages of total words masked under different masking policies for the American English speaker in each mask split across both test sets.}
  \centering
  \begin{tabular}{ lccccc }
    &\multicolumn{3}{c}{\textbf{Mask Nouns}}&\multicolumn{2}{c}{\textbf{Mask All}}\\
    %\% of instruction 
    Mask proportion &\textit{20\%}&\textit{40\%}&\textit{100\%}&\textit{20\%}&\textit{40\%}\\
    %%% SINGLE DECIMAL PRECISION %%%
    \toprule
    Test (\textit{seen}) & 9.6\% & 15.8\% & 29.3\% & 23.1\% & 42.3\%\\
    Test (\textit{unseen}) & 9.5\% & 15.6\% & 29.0\% & 23.1\% & 42.3\%\\
    \bottomrule
  \end{tabular}
  \label{tab:mask_counts}
\end{table}

==> Sections/contributions.tex <==
Our main contributions are as follows:
(1) We present empirical evidence that multimodal speech recognition outperforms unimodal methods on noisy audio in an embodied agent context;
\todo{(2) We analyze how visual information is utilized in the multimodal approach;}
\todo{(3) We analyze the error propagation from speech recognition to action selection of agents;}
\todo{(4) We demonstrate the accuracy improvement of a speech recognition re-ranker on a constrained domain.}
